Contrastive Learning for Sequential Recommendation

Sequential recommendation methods play a crucial role in modern recommender systems because of their ability to capture a user's dynamic interest from her/his historical interactions. Despite their success, we argue that these approaches usually rely on the sequential prediction task to optimize the huge amounts of parameters. They usually suffer from the data sparsity problem, which makes it difficult for them to learn high-quality user representations. To tackle that, inspired by recent advances of contrastive learning techniques in the computer version, we propose a novel multi-task model called \textbf{C}ontrastive \textbf{L}earning for \textbf{S}equential \textbf{Rec}ommendation~(\textbf{CL4SRec}). CL4SRec not only takes advantage of the traditional next item prediction task but also utilizes the contrastive learning framework to derive self-supervision signals from the original user behavior sequences. Therefore, it can extract more meaningful user patterns and further encode the user representation effectively. In addition, we propose three data augmentation approaches to construct self-supervision signals. Extensive experiments on four public datasets demonstrate that CL4SRec achieves state-of-the-art performance over existing baselines by inferring better user representations.

==> related.tex <==
\section{Related Work}
In this section, we will review previous works related to ours in two aspects, including sequential recommendation and self-supervised learning.
\subsection{Sequential Recommendation}
Early works on sequential recommendations usually utilize the theory of Markov Chain~(MC) to capture sequential patterns from successive item sequences. 
For example, \citeauthor{FPMC}~\cite{FPMC} combine first-order MC and matrix factorization to capture both the smoothness of subsequent actions and long-term user preference~(FPMC). 
Besides the first-order MCs, there are also methods adopting high-order MC, which consider more preceding items to extract more complicated sequential patterns~\cite{Fossil,Vista}.

With the recent advance of deep learning, there are many works that are equipped with these powerful tools and achieve significant breakthrough in sequential recommendation tasks~\cite{DREAM,GRU4Rec,caser,SASRec,Fossil,SUM,UserGRU,Future, 2DCNN}.
Recurrent neural networks~(RNN)~\cite{RNN} and its variants, such as Long Short-Term Memory~(LSTM)~\cite{LSTM} and Gated Recurrent Unit~(GRU)~\cite{GRU}, which are designed for sequential data, \zyrm{are appropriate to model user behavior sequences.} \zhaoyang{are applied for user behavior sequences.}
For example, \citeauthor{GRU4Rec}~\cite{GRU4Rec} firstly adopt GRU modules to the session-based recommendation task with ranking loss.
The following variants modified GRU4Rec by introducing attention mechanism~\cite{NARM,AIR,SDM}, hierarchical structure~\cite{Hierarchical}, user-based GRU~\cite{UserGRU}.%

Other deep learning models are also adopted to sequential recommendation tasks and achieve excellent performance. 
For instance, \citeauthor{caser}~\cite{caser}  propose a Convolutional Sequence
Embedding Recommendation Model~(Caser) to learn sequential
patterns as local features of the ``image'' using both horizontal and vertical convolutional filters. 
\citeauthor{SUM}~\cite{SUM} and \citeauthor{Memeory}~\cite{Memeory} leverage the memory-augmented neural network~(MANN) to store and update useful information explicitly.
HGN~\cite{HGN} captures both the long-term and short-term user interest by introducing a hierarchical gating network including a feature gating module, an instance gating
module, and an item-item product module.

Recently, the self-attention network~\cite{Transformer} has shown promising potential in modeling sequential data.
Inspired by this mechanism, \citeauthor{SASRec}~\cite{SASRec} utilize Transformer layers to adaptively assign weights to previous items in the sequential recommendation task.
\citeauthor{Bert4rec}~\cite{Bert4rec} improve that by adopting a bidirectional Transformer to incorporate user behaviors information from both directions, since the user’s historical interactions may not be a rigid order~\cite{Rigidorder}.

In recent years, GNN~\cite{GNN} has aroused comprehensive attention in the deep learning society.
Since GNN can capture complicated item transition patterns hidden in user sequences, many works attempt to utilize powerful GNN techniques in sequential recommendation tasks, especially when user sequences are short anonymous sessions.
For example, \citeauthor{SRGNN}~\cite{SRGNN} adopt the gated graph network to aggregate the neighborhood information and make adjustment for the directed graph.
Later, \citet{FGNN} utilize attention mechanism as the aggregation function to differentiate the influence of different neighbors, instead of mean pooling.
To capture both global and local structure, ~\citet{GCSAN} combine self-attention with GNN and achieve promising results for the session-based recommendation.





\subsection{Self-supervised Learning}
Self-supervised learning has aroused comprehensive awareness recently, since it concentrates on learning useful representations from unlabeled data, which benefits the downstream tasks. 
Its basic idea is to construct training signals by designing pretext tasks within the raw data and then utilize them to train the model.
The pretext tasks usually transform the raw data into another near-equivalent form and then predict the details of the transformation (\textit{prediction task}) or distinguish whether samples are transformed from the same data (\textit{discrimination task}). 

The prediction tasks have been widely adopted in CV and NLP.
In the CV community, various self-supervised learning pretext tasks have been widely exploited~\cite{Revisit_cvpr}, such as predicting image rotations~\cite{Image_rotation}, predicting relative patch locations~\cite{relative_patch}, solving jigsaw puzzles~\cite{Jigsaw}, and solving colorization problems~\cite{Colorization}.
When it comes to the area of NLP, many works are focusing on self-supervised techniques to acquire universal word representations.
The language model is a popular self-supervised objective in this area that learns to predict the next word given the previous words~\cite{Language_Model}.
There are also other pretext tasks in the NLP area, such as the Cloze task and next sentence prediction, and so on~\cite{BERT,GPT-2}. 
Though these prediction tasks have achieved promising results, they rely on ad-hoc heuristics, which may affect the generality of the representations~\cite{Simclr}.

In contrast, the discrimination tasks adopt a contrastive learning technique that tries to distinguish the positive sample from massive negative samples in a classification manner.
\citeauthor{Memory_bank}~\cite{Memory_bank} claims that the use of rich negative samples can enhance the performance of contrastive learning, so they propose an approach to sample negative instances from a shared memory bank.
Later, \citeauthor{Momentum_contrast}~\cite{Momentum_contrast} equip the memory bank with a dynamic queue and a moving-averaged encoder to build large and consistent dictionaries.
There are also other works that exploit the use of in-batch negative samples rather than a memory bank~\cite{In-sample,Simclr}.

When it comes to the field of recommendation systems, some works apply self-supervised learning to improve recommendation performance.
For example, \citeauthor{RL_supervised}~\cite{RL_supervised} propose Self-Supervised Q-learning~(SQN) and Self-Supervised Actor-Critic~(SAC) to consider long-term user engagement using multiple types of users' behaviors.
\citeauthor{Google}~\cite{Google} present a self-supervised learning framework to learn useful representations of items that have a set of categorical features.
Later, \citeauthor{S3}~\cite{S3} design auxiliary self-supervised objectives to learn the correlations among attribute, item, subsequence, and sequence.
Different from the above methods, our model focuses on how to learn useful user representations just from a single type of users' behaviors without auxiliary information.







